Deep Slice Interpolation via Marginal Super-Resolution, Fusion and Refinement

We propose a marginal super-resolution (MSR) approach based on 2D convolutional neural networks (CNNs) for interpolating an anisotropic brain magnetic resonance scan along the highly under-sampled direction, which is assumed to axial without loss of generality. Previous methods for slice interpolation only consider data from pairs of adjacent 2D slices. The possibility of fusing information from the direction orthogonal to the 2D slices remains unexplored. Our approach performs MSR in both sagittal and coronal directions, which provides an initial estimate for slice interpolation. The interpolated slices are then fused and refined in the axial direction for improved consistency. Since MSR consists of only 2D operations, it is more feasible in terms of GPU memory consumption and requires fewer training samples compared to 3D CNNs. Our experiments demonstrate that the proposed method outperforms traditional linear interpolation and baseline 2D/3D CNN-based approaches. We conclude by showcasing the method's practical utility in estimating brain volumes from under-sampled brain MR scans through semantic segmentation.

==> 1slice_vs_3slice/1slice_vs_3slice_graph.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[height=1in]{1slice_vs_3slice/cor_est_1slice.png}
        \caption{}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[height=1in]{1slice_vs_3slice/sag_est_1slice.png}
        \caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[height=1in]{1slice_vs_3slice/cor_est_3slice.png}
        \caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[height=1in]{1slice_vs_3slice/sag_est_3slice.png}
        \caption{}
    \end{subfigure}
    \caption{Comparison of 1 slice vs 3 slices as input}    
\end{figure*}

==> ablation/GAN_vs_noGAN.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in]{ablation/GAN_vs_noGAN/refined_L1.png}
        \caption{Refined, L1}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[height=1.5in]{ablation/GAN_vs_noGAN/refined_GAN.png}
        \caption{Refined, L1+GAN}
    \end{subfigure}
    \caption{Comparison of refined image, with and without GAN loss.}    
\end{figure*}

==> comparison/comparison.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.125\textwidth}
        \caption{LI}
        \centering
        \includegraphics[width=\linewidth]{comparison/img1/LI_box.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \caption{2D CNN}
        \centering
        \includegraphics[width=\linewidth]{comparison/img1/2frames_box.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \caption{3D CNN}
        \centering
        \includegraphics[width=\linewidth]{comparison/img1/3DSR_box.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \caption{Ours}
        \includegraphics[width=\linewidth]{comparison/img1/3slices_box.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \caption{Ground Truth}
        \includegraphics[width=\linewidth]{comparison/img1/HR_box.png}
    \end{subfigure}
    
    \vspace{-2em}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img1/LI_region.png}
        \vspace{-2em}
        \caption{\tiny{25.51/0.7681}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img1/2frames_region.png}
        \vspace{-2em}
        \caption{\tiny{28.29/0.8205}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img1/3DSR_region.png}
        \vspace{-2em}
        \caption{\tiny{29.51/0.8824}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img1/3slices_region.png}
        \vspace{-2em}
        \caption{\tiny{31.87/0.9249}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img1/HR_region.png}
        \vspace{-2em}
        \caption{\tiny{PSNR(dB)/SSIM}}
    \end{subfigure}        
    
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/LI_box.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/2frames_box.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/3DSR_box.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/3slices_box.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/HR_box.png}
    \end{subfigure}
    
    \vspace{-2em}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/LI_region.png}
        \vspace{-2em}
        \caption{\tiny{23.78/0.6866}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/2frames_region.png}
        \vspace{-2em}
        \caption{\tiny{27.38/0.8180}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/3DSR_region.png}
        \vspace{-2em}
        \caption{\tiny{27.21/0.8128}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/3slices_region.png}
        \vspace{-2em}
        \caption{\tiny{29.52/0.8755}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img2/HR_region.png}
        \vspace{-2em}
        \caption{\tiny{PSNR(dB)/SSIM}}
    \end{subfigure}       
    
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/LI_box.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/2frames_box.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/3DSR_box.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/3slices_box.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/HR_box.png}
    \end{subfigure}
    
    \vspace{-2em}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/LI_region.png}
        \vspace{-2em}
        \caption{\tiny{27.37/0.8465}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/2frames_region.png}
        \vspace{-2em}
        \caption{\tiny{32.34/0.9441}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/3DSR_region.png}
        \vspace{-2em}
        \caption{\tiny{32.72/0.9436}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/3slices_region.png}
        \vspace{-2em}
        \caption{\tiny{34.11/0.9607}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \centering
        \includegraphics[width=\linewidth]{comparison/img3/HR_region.png}
        \vspace{-2em}
        \caption{\tiny{PSNR(dB)/SSIM}}
    \end{subfigure}      
    
    \caption{Visual Comparison of Linearly Interpolation and CNN based methods (top two from X8, bottom example from X4).}    
\end{figure*}

==> global_context/global_context.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[height=1in]{global_context/input.png}
        \caption{Input, 16X degradation}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[height=1in]{global_context/L1GAN_32_32.png}
        \caption{Patch-wise SR with GAN}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[height=1in]{global_context/L1GAN_256_256.png}
        \caption{Image-wise SR with GAN}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[height=1in]{global_context/gt.png}
        \caption{Ground Truth}
    \end{subfigure}
    \caption{Comparison of medical image SR with and without global context}    
\end{figure*}

==> global_context/text.tex <==
\subsubsection{The importance of global context}

We like motivate our work by briefly demonstrating the importance of global context in medical imaging. 

Unlike natural images, which vary sporadically from each other, medical images usually have very consistent structures. Although training on small patches has been a standard practice with current state-of-the-art SISR methods on natural images, it strips of network's ability to extract a general global structure, which exists with medical images. As a consequence, 

A toy demonstration is shown in Fig. 3, where we attempt to up-sample a severely downgraded image through a RDN. Due to the bad quality of the input, we use GAN loss to help generate reasonable information. As we can see from the images, when training with patches, the discriminator network cannot locally distinguish the differences between brain and mouth tissue, therefore driving the generator to create similar structures without being penalized. On the other hand, if we train with the entire brain image, the discriminator is able to find a global structure and does a much better job at generating structurally coherent images, where brain and mouth tissues are not the same.

This conclusion motivates us to find ways that can avoid patch-wise training, especially when GAN is involved. 
